DETER: Detecting Edited Regions for Deterring Generative Manipulations

Generative AI capabilities have grown substantially in recent years, raising renewed concerns about potential malicious use of generated data, or "deep fakes". However, deep fake datasets have not kept up with generative AI advancements sufficiently to enable the development of deep fake detection technology which can meaningfully alert human users in real-world settings. Existing datasets typically use GAN-based models and introduce spurious correlations by always editing similar face regions. To counteract the shortcomings, we introduce DETER, a large-scale dataset for DETEcting edited image Regions and deterring modern advanced generative manipulations. DETER includes 300,000 images manipulated by four state-of-the-art generators with three editing operations: face swapping (a standard coarse image manipulation), inpainting (a novel manipulation for deep fake datasets), and attribute editing (a subtle fine-grained manipulation). While face swapping and attribute editing are performed on similar face regions such as eyes and nose, the inpainting operation can be performed on random image regions, removing the spurious correlations of previous datasets. Careful image post-processing is performed to ensure deep fakes in DETER look realistic, and human studies confirm that human deep fake detection rate on DETER is 20.4% lower than on other fake datasets. Equipped with the dataset, we conduct extensive experiments and break-down analysis using our rich annotations and improved benchmark protocols, revealing future directions and the next set of challenges in developing reliable regional fake detection models.

==> sec/0_abstract.tex <==

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=1.0\textwidth]{figs/figure1_v2.pdf}
%     % \vspace{-0.25in}
%     \caption{\textbf{In this work, we introduce \emph{ReFA} dataset for the regional fake detection task with human analysis.} By formalizing the problem as a regional segmentation task, models can achieve much better detection performance, while we humans and popular Large Language Models (LLMs) (i.e., GPT-4~\cite{OpenAI_ChatGPT}) usually fail to distinguish the differences.}
%     \label{fig:teaser}
%     % \vspace{-0.1in}
% \end{figure*}



\begin{abstract}
%V1
% With the recent booming of Generative AI, concerns regarding the potential malicious usage of deep generative models and their generated fake data have reached their zenith. 
% In this work, we introduce the \textbf{ReFA}, featuring an up-to-date, high-quality and comprehensive image dataset for \textbf{Re}gional \textbf{F}ake detection with IRB (Institutional Review Boards) approved human \textbf{A}nalysis.
% \textbf{ReFA} includes 300,000 high-resolution images edited by four state-of-the-art generators based on GANs and Diffusion Models, integrates three different editing operations in diverse granularities (i.e., face swapping, face inpainting, and face attribute editing) with precise pixel-level mask annotations, and incorporates realistic visual scenarios with both single and multiple faces settings.
% Unlike most existing deepfake datasets of static images extracted from videos with true or false labels, our dataset enables versatile image-level downstream applications, ranging from classic binary classification to challenging regional fake mask predictions. 
% Accordingly, we cast the regional fake detection task as a fine-grained region detection problem to tackle the problem, and benchmark extensive segmentation models with various metrics.  
% Last but not least, we note the special nature of regional fake detection, and propose to bring human evaluations and analysis to supplement the conventional automatic evaluation systems and to provide novel insights for supporting future human-centric and responsible AI studies~\footnote{\emph{ReFA} will be publicly released upon acceptance.}.



%V2
% With the recent booming of Generative AI, concerns regarding the potential malicious usage of deep generative models and their generated fake data have reached their zenith. 
% In this work, we introduce the \textbf{ReFA}, featuring an up-to-date, high-quality and comprehensive image dataset for \textbf{Re}gional \textbf{F}ake detection with IRB (Institutional Review Boards) approved human \textbf{A}nalysis.
% \textbf{ReFA} includes 300,000 high-resolution images edited by four state-of-the-art generators based on GANs and Diffusion Models, integrates three different editing operations in diverse granularities with annotations from versatile dimensions (i.e., images, masks, generative models, operations), and incorporates realistic visual scenarios with both single and multiple faces settings.
% We seek to ground and bridge the related research communities from the following three perspectives: 
% For the detection side, we cast the regional fake detection task as a fine-grained region detection problem to tackle the problem, and benchmark extensive segmentation models with multiple classic metrics. 
% For the generative side, we show that a step forward beyond the current visual photorealistic goal could be deep-feature similarities via our deep-dive model-wise empirical analysis. 
% Last but not least, we investigate the role of humans in this adversarial game by bringing human evaluations and analysis to provide novel insights to supplement the conventional automatic evaluations for supporting future human-centric and responsible AI studies~\footnote{\emph{ReFA} will be publicly released upon acceptance.}.


%V3

With the recent booming of Generative AI, concerns regarding the potential malicious usage of deep generative models and their generated fake data have reached their zenith. 
In this work, we introduce the \textbf{ReFA}, featuring an up-to-date, high-quality and comprehensive image dataset for \textbf{Re}gional \textbf{F}ake detection with IRB (Institutional Review Boards) approved human \textbf{A}nalysis.
\textbf{ReFA} includes 300,000 images edited by four state-of-the-art generators based on GANs and Diffusion Models, integrates three different editing operations in diverse granularities with annotations from multiple axes (i.e., images, masks, generative models, operations), and incorporates realistic visual scenarios with both single and multiple faces settings.
Unlike most existing deepfake datasets of static images extracted from videos with true or false labels, our dataset enables versatile image-level downstream applications, ranging from classic binary classification to challenging regional fake mask predictions. 
Accordingly, we cast the regional fake detection task as a fine-grained region detection problem to tackle the problem, and benchmark extensive segmentation models with various metrics.
Last but not least, we note the special nature of regional fake detection, and propose to bring human evaluations and analysis to supplement the conventional automatic evaluation systems and to provide novel insights for supporting future human-centric and responsible AI studies~\footnote{\emph{ReFA} will be publicly released upon acceptance. We also conduct the same evaluation tests with LLMs~\cite{OpenAI_ChatGPT}, details in the Appendix~\ref{app_sec:llms}.}.



% we perform supplementary human studies to promote the alignment between conventional modeling based automatic evaluations and human based evaluations. 


\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Para1: Why do we introduce this, the need for deep fake detection, regional deep fake detection, and a high-quality benchmark
% Para2: Dataset: what differs us from existing datasets
% Para3: Modeling:
% Para4: Human insights

\textit{``If you know both enemy and yourself, you will fight a hundred battles without danger or failure."} 

\textit{\hfill -- Sun Tzu, The Art of War, 300 BC}


\begin{figure}[t]
\centering\includegraphics[width=0.45\textwidth]{figs/figure0.pdf}
    \caption{Generative AI techniques are rapidly shaping our real life.}
    \label{fig:idea}
\end{figure}

Generative AI has captured significant attention from both the computer vision research community and the general public in recent years, following groundbreaking advances in generative modeling.
The booming of those generative AI techniques brings numerous advantages and conveniences but also raises heightened concerns about the potential malicious usage of their generated fake data, especially within the context of identifiable human faces. 
As a protective shield against the potential misuse of generative AI techniques, the research on fake detection has long been a significant direction but has also often been relatively detached from its counterpart in terms of datasets, benchmarks and evaluations.   
Our primary motivation in this work is to catch up with the rapidly advancing generative techniques for an effective protective strategy, by bridging both the generative and detection sides.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/figure1_v3.pdf}
    \caption{\textbf{In this work, we introduce \emph{ReFA} dataset for the regional fake detection task with human analysis.} By formalizing the problem as a regional segmentation task, models can achieve much better detection performance, while we humans and popular Large Language Models (LLMs) (i.e., GPT-4~\cite{OpenAI_ChatGPT}) usually fail to distinguish the differences.}
    \label{fig:teaser}
    % \vspace{-0.1in}
\end{figure*}


\emph{First}, in the upstream generative architecture area, the Diffusion Models (DMs)~\cite{sohl2015dpm_thermo,ho2020dpm,theo-diff2} are gradually replacing Generative Adversarial Nets (GANs)~\cite{gan,karras2017progressive,gal2022stylegan} and become the new state-of-the-art generative models by achieving impressive performance in data generation for images~\cite{stablediff,dhariwal2021diff-img1,ho2022diff-img2,song2020ddim,ramesh2022dalle2,ho2022imagen}, audio~\cite{kong2020diffwave,zhu2022discrete,mittal2021symbolic-diff,lee2021nu}, and videos~\cite{ho2022video,singer2022make}.
On the downstream front, where generative models are leveraged for versatile and fine-grained applications like data editing and customization, both GANs-based~\cite{liu2023fine,yildirim2023diverse,li2022mat,pan2023drag} and DMs-based frameworks~\cite{zhu2023boundary,kim2022diffusionclip,liu2023flowgrad,ruiz2023dreambooth,yang2023diffusion} continue to share an equal footing.
However, as listed in Table~\ref{tab:datasets}, most existing deep fake datasets~\cite{rossler2018faceforensics,rossler2019faceforensics++,li2020celeb,zi2020wilddeepfake,korshunov2018deepfakes,yang2019exposing,dolhansky2019deepfake,jiang2020deeperforensics1,he2021forgerynet} are mainly \emph{video-based}, which misaligns with the current trend in generative modeling area for high-resolution image synthesis and manipulations~\cite{ramesh2022dalle2,ho2022imagen,dhariwal2021diff-img1,stablediff}.
Also, the majority of them come from classic but relatively outdated generative backbones (mostly Autoencoder and GANs based~\cite{korshunov2018deepfakes,he2021forgerynet}), or unspecified model sources with Computer Graphics techniques and existing software applications~\cite{li2020celeb,zhou2017two} in terms of generators.
Failure to catch up with the fast-developing generative fields in the dataset construction front sets the first gap between the generative and detection teams.
Specifically, recent literature suggests that despite the seemingly similar visual effects in terms of image editing, GANs~\cite{gan} and DMs~\cite{sohl2015dpm_thermo,ho2020dpm} work in evidently different modeling mechanisms, which leads to distinguishable latent spectrum~\cite{corvi2023detection,ricker2022towards}.
To this end, our \emph{ReFA} presents high-quality images edited by four state-of-the-art generators (at most one-year long) based on both GANs and DMs backbones~\cite{xia2023diffir,li2022mat,zhao2023diffswap,liu2023e4s}.
This is also the first large-scale regional deepfake dataset with DMs-based generators to the best of our knowledge.
More details about our \emph{ReFA} dataset are presented in Sec.~\ref{sec:dataset}.
% and Appendix~\ref{app_sec:dataset}.

\begin{table*}[th]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{l|ccccccc}
    \toprule
       Datasets  & Original Format & Real & Fake & Generators & Operations & Annotations & Multiple Faces \\ \hline \hline
       DF-TIMIT 18'~\cite{korshunov2018deepfakes} & Videos & 320 & 640 & GANs & Swap & Binary & -  \\
        FaceForensics++ 19'~\cite{rossler2019faceforensics++}& Videos & 1,000 & 5,000 & AEs/CG & Swap & Binary/Masks  & -\\
       Celeb-DF 20'~\cite{li2020celeb} & Videos & 590 & 5,639 & AEs/GANs & Swap & Binary & -\\
       DFFD 20'~\cite{dang2020detection} & Videos & 1,000 & 3,000 & AEs/GANs & Swap/Attribute. & Binary/Masks  & -\\
       DFDC 20'~\cite{dolhansky2020dfdc} & Videos & 23,564 & 104,500 & GANs/AEs/CG & Swap & Binary  & - \\
       ForgeryNet 21'~\cite{he2021forgerynet} & Videos & 99,630 & 121,617 & GANs & Swap/Attribute & Binary/Masks  & Contained \\
       SwapMe/FaceSwap 17'~\cite{zhou2017two} & Images & 4,600 & 2,010 & CG/App. & Swap & -  & - \\ 
       OpenForensics 21'~\cite{le2021openforensics} & Images & 45,473 &  115,325 & GANs & Swap & Binary/Masks  & Contained \\
       % DGM$^4$ 23'~\cite{shao2023detecting} & Images\&Texts & 77,426 &  152,574 & GANs & Swap/Attribute & Binary/Box/Edit\\
       \hline
        ReFA (Ours) & Images & 38,996 &300,000 & GANs/DMs & Swap/Inpaint/Attribute & Binary/Masks/Models/Edit & Contained \\ 
    \bottomrule
    \end{tabular}}
    % \vspace{-0.1in}
    \caption{\textbf{Comparison of basic dataset statistics for deepfake detection.} We list the existing popular deepfake datasets in time ordering, with their scales, generators and editing operations. Most existing popular deepfake datasets are video-based, several recent image datasets edit the face images with the swapping operation. \emph{ReFA} includes the state-of-the-art GANs and DMs-based generators with diverse editing and annotations.}
    \label{tab:datasets}
    % \vspace{-0.1in}
\end{table*}

% The booming of those generative AI techniques brings numerous advantages and conveniences, but also raises more concerns on the potential malicious usage of their generated fake data than ever before, especially within the context of identifiable human faces.  


% Existing dataset: lack 1 - comprehensive of generators (either GAN & Diffusion based)/ - over-simplified task settings (binary) and evaluations
% As a protective shield against generative AI techniques for potential malicious usage, the research on fake detection has long been a significant direction but has often lagged behind and struggles to catch up with its generative counterpart. 
% We note that the absence of an up-to-date, high-quality and comprehensive dataset, as well as over-simplified task formulations and evaluations are critical causes for this gap.

% \emph{First}, most existing deep fake datasets~\cite{rossler2018faceforensics,rossler2019faceforensics++,li2020celeb,zi2020wilddeepfake,korshunov2018deepfakes,yang2019exposing,dolhansky2019deepfake,jiang2020deeperforensics1,he2021forgerynet} are mainly video-based with relatively low resolutions, which misaligns with the current trend in generative modeling for high-resolution image synthesis~\cite{ramesh2022dalle2,ho2022imagen,dhariwal2021diff-img1,stablediff}.
% Also, the majority of them come from a single generative backbone (mostly GAN-based~\cite{korshunov2018deepfakes,he2021forgerynet}) or even unspecified source~\cite{li2020celeb} in terms of generators.
% However, up-to-date and comprehensive sources of the generators in a deepfake dataset are crucial for fake detection studies as ``if you know both the enemy and yourself, you will fight a hundred battles without danger of defeat''~\footnote{Quote from the \emph{The Art of War} by Sun Tzu, around 300 B.C.}.
% Specifically, despite the seemingly similar visual effects in terms of image editing, GANs~\cite{gan} and DMs~\cite{sohl2015dpm_thermo,ho2020dpm} work in dramatically different modeling mechanisms, which leads to distinguishable latent spectrum~\cite{corvi2023detection,ricker2022towards}. 
% Failure to catch up with the fast-developing generative fields in the dataset construction front sets the first step behind for the detection side.
% To this end, our \emph{ReFA} presents high-quality images edited by four state-of-the-art generators (at most one-year long) based on both GANs and DMs backbones~\cite{xia2023diffir,li2022mat,zhao2023diffswap,liu2023e4s}, in (xx resolutions). More details about our \emph{ReFA} dataset are presented in Tab.~\ref{tab:datasets}, Sec.~\ref{sec:dataset} and Appendix~\ref{app_sec:dataset}.


\emph{Second}, current works often formalize the image-level fake detection problem as a binary classification task~\cite{wang2023dire,corvi2023detection,ricker2022towards}, underestimating the fine-grained editing generators~\cite{zhao2023diffswap,liu2023e4s} and over-simplifying the real-life malicious scenarios where often part of the real images are modified without changing the personal identity (e.g., the change of hair color or styles can leads to wrong judgment on the time testimony, see examples from our dataset in Fig.~\ref{fig:teaser}).
Moreover, as for the deepfake detection, we would not only want the protective AI models to predict a binary label given a potentially modified image, but an intuitive step forward would be more fine-grained region prediction from detection frameworks.
A few recent image datasets such as OpenForensics~\cite{le2021openforensics} are proposed for this purpose with mask annotations, however, it covers only the face swaping editing operation.
To address the above concerns, we integrate three editing operations in different granularities (i.e., face swapping, face inpainting, and attribute editing, ordering from coarse to fine), each annotated with image binary labels, precise masks and source generators.
Accordingly, we cast the fake detection problem as a more challenging and fine-grained segmentation task, asking the detection models to predict pixel-level regions that are likely to be changed by deep generators.
Extensive evaluations in terms of classic automatic metrics are reported in Sec.~\ref{sec:detection}.
% and Appendix~\ref{app_sec:detection}. 
Note that the scale of our \emph{ReFA} (300K) is on par or superior compared to classic large-scale object detection and segmentation benchmarks such as MSCOCO ($\sim$330K)~\cite{lin2014microsoft}, LVIS ($\sim$164K)~\cite{gupta2019lvis}, and ADE20K ($\sim$27K)~\cite{zhou2017scene}.


\emph{Last but certainly not least}, AI has entered an era where its techniques are no longer confined to the research community; instead, they are rapidly and profoundly shaping human life.
However, despite the common recognition that our research should consider the potential social and human applications, particularly in the context of sensitive areas like deepfake detection, where humans are integral to both data content and real-world user cases, existing literature has seldom incorporated comprehensive human studies and analysis in either datasets~\cite{he2021forgerynet} and detection modeling~\cite{wang2023dire,corvi2023detection,ricker2022towards}. 
To fill the current gap and raise awareness of this overlooked human factor, we conduct IRB-approved human studies with two specific layouts that align with the current automatic evaluations to supplement the conventional evaluation protocols, specified in Sec.~\ref{sec:human}. 
While humans are usually believed to be the performance upper-bound in various computer vision tasks to ground the model learning such as object recognition and segmentation~\cite{zhao2019object,minaee2021image}, they become \emph{lower-bound} in fake detection, which further confirms the great potential and necessity of model assistance when deploying Generative AI in real life.
% We also reveal that XXXX via further error pattern analysis, shed light on the novel perspective to re-think the fake detection problem. 








% Human study
% Particularly, the fake detection problem that closely embedded with human perception, yet none of existing dataset or detection modeling works have ever considered the problem from the  


% Summary
To sum up, the contributions of our work can be categorized into the following three aspects:
\begin{itemize}
    \item We introduce the \emph{ReFA} dataset, featuring an up-to-date, high-quality, and comprehensive image dataset for regional fake detection with diverse annotations from different dimensions such as binary image labels, editing masks, generative models and operations. 
    % Our primary goal is to catch up with the generative modeling side to build 
    \item We formalize the regional fake detection problem as a fine-grained segmentation task, and conduct extensive experiments with various evaluation metrics to establish a comprehensive benchmark.
    \item We conduct IRB approved human studies and analysis in terms of fake detection evaluations, providing insights for supporting future human-centric studies from this commonly overlooked perspective.
    % ~\footnote{We also conduct the same evaluation tests with LLMs (i.e., GPT4), more details and insights are included in Appendix~\ref{app_sec:llms}.
    % }
\end{itemize}










% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related}

We present existing literature from domains that are mostly closely related to our work in this section.


\noindent \textbf{Deepfake Datasets.}
Most existing popular deepfake datasets~\cite{rossler2018faceforensics,rossler2019faceforensics++,li2020celeb,zi2020wilddeepfake,korshunov2018deepfakes,yang2019exposing,dolhansky2019deepfake,jiang2020deeperforensics1,he2021forgerynet,dang2020detection} are video-based, with several of them providing static images extracted from video clips~\cite{he2021forgerynet,dang2020detection}.
While the video-based datasets indeed present valuable challenges in downstream applications such as the temporal forgery localization task~\cite{he2021forgerynet}, we note that the current mainstream modeling works in the generative field are still focusing on image-level manipulations such as semantic editing~\cite{kim2022diffusionclip,kwon2022diffusion,zhu2023boundary} and  inpainting~\cite{li2022mat,xia2023diffir,lugmayr2022repaint}.   
Given our goal to align with the fast developing generative side and build a protective shield against those deep generators, we present an image dataset that uses the latest state-of-the-art fine-grained methods as generators, and covers several mainstream editing operations with different granularities.



\noindent \textbf{Generative Models for Image Manipulations.}
While diffusion models (DMs)~\cite{sohl2015dpm_thermo,ho2020dpm,theo-diff1,theo-diff2,stablediff,ramesh2022dalle2,dhariwal2021diff-img1} are steadily replacing generative adversarial networks (GANs)~\cite{gan,karras2017progressive,gal2022stylegan,xu2018attngan} and have become the novel dominating method for image synthesis in the past two years, the latter has not yet been entirely supplanted in the downstream side for more fine-grained applications such as image manipulation. 
Among the most recent works that perform fine-grained image manipulations within the past two years~\cite{liu2023fine,yildirim2023diverse,li2022mat,pan2023drag,liu2023e4s,zhao2023diffswap,zhu2023boundary,kwon2022diffusion,lugmayr2022repaint,xia2023diffir}, we carefully select four methods~\cite{liu2023e4s,li2022mat,zhao2023diffswap,xia2023diffir} that cover both GANs and DMs backbones based on their editing quality and versatility as the generators in this work.  


% \begin{table*}[th]
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{l|ccccccc}
%     \toprule
%        Datasets  & Original Format & Real & Fake & Generators & Operations & Annotations \\ \hline \hline
%        DF-TIMIT 18'~\cite{korshunov2018deepfakes} & Videos & 320 & 640 & GANs & Swap & Binary  \\
%         FaceForensics++ 19'~\cite{rossler2019faceforensics++}& Videos & 1,000 & 5,000 & AEs/CG & Swap & Binary/Masks\\
%        Celeb-DF 20'~\cite{li2020celeb} & Videos & 590 & 5,639 & AEs/GANs & Swap & Binary \\
%        DFFD 20'~\cite{dang2020detection} & Videos & 1,000 & 3,000 & AEs/GANs & Swap/Attribute. & Binary/Masks\\
%        DFDC 20'~\cite{dolhansky2020dfdc} & Videos & 23,564 & 104,500 & GANs/AEs/CG & Swap & Binary  \\
%        ForgeryNet 21'~\cite{he2021forgerynet} & Videos & 99,630 & 121,617 & GANs & Swap/Attribute & Binary/Masks\\
%        SwapMe/FaceSwap 17'~\cite{zhou2017two} & Images & 4,600 & 2,010 & CG/App. & Swap & -\\ 
%        % DiffusionForensics 23'~\cite{wang2023dire} & Images &  \\
%        \hline
%         ReFA (Ours) & Images & 38,996 &300,000 & GANs/DMs & Swap/Inpaint/Attribute & Binary/Masks \\ 
%     \bottomrule
%     \end{tabular}}
%     \caption{\textbf{Comparison of dataset statistics for deepfake detection.} We list the existing popular deepfake datasets in time ordering, with their scales, generators and editing operations.}
%     \label{tab:datasets}
% \end{table*}



\noindent \textbf{Fake Detection Modeling.}
Fake detection methods are closely entangled with available datasets and evaluation systems.
Many earlier works~\cite{liu2020global,dang2020detection,li2020face,wang2020cnn,yu2019attributing} tackle the problem against GAN-based generators using Convolutional Neural Networks (CNNs) discriminators and can already achieve very high accuracy (more than 99.9\%) in discerning fake/real images. 
Even the most recent fake detection works that build upon diffusion models~\cite{corvi2023detection,ricker2022towards,wang2023dire} still follow the conventional setting and formalize it as a binary classification problem. 
However, the demand for fake detection methods has gone beyond a true or false label, especially given the more sophisticated generators.
In this work, we take a step forward on the modeling and formalize the problem as a more fine-grained segmentation task. 

% \begin{figure*}[th]
%     \centering    \includegraphics[width=0.8\textwidth]{figs/figure2_v2.pdf}
%     \caption{\textbf{Pipeline for our regional fake approach.} We first pre-process the real images with face detection and mask parsing techniques~\cite{bulat2017far,yu2021bisenet}. Next, we provide different binary masks as well as the detected face regions (also optional reference images if necessary for swapping and attribute editing operations) as the input to selected SOTA generators to obtain edited regions in different granularities. Finally, we apply a series of post-rendering techniques and paste the edited regions back to original images, ensuring high visual quality of the edited images in our dataset. \ye{This figure may need further change/improvement.}}
%     \label{fig:pipeline}
%     % \vspace{-0.1in}
% \end{figure*}

%citations: gabriel2020artificial, global
\noindent \textbf{Humans in Fake Detection.}
The human perspective has been an increasingly important yet often overlooked factor in modern AI studies. 
In the literature of deepfake detection, relatively few previous works have integrated human studies either in datasets or modeling. FaceForensics++~\cite{rossler2019faceforensics++} compares the manual and automatic settings on video forgery detection. 
Liu \textit{et al.}~\cite{liu2020global} investigate the human performance on image fake detection.
Both above works ask human participants to distinguish fake or true data, which aligns with the mainstream formulation of binary classification.
In our work, we perform IRB approved human studies not only on the classification level but also more fine-grained regional detection analysis.






% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.
